Towards Computer-Vision Based Vineyard Navigation for Quadruped Robots

There is a dramatic shortage of skilled labor for modern vineyards. The Vinum project is developing a mobile robotic solution to autonomously navigate through vineyards for winter grapevine pruning. This necessitates an autonomous navigation stack for the robot pruning a vineyard. The Vinum project is using the quadruped robot HyQReal. This paper introduces an architecture for a quadruped robot to autonomously move through a vineyard by identifying and approaching grapevines for pruning. The higher level control is a state machine switching between searching for destination positions, autonomously navigating towards those locations, and stopping for the robot to complete a task. The destination points are determined by identifying grapevine trunks using instance segmentation from a Mask Region-Based Convolutional Neural Network (Mask-RCNN). These detections are sent through a filter to avoid redundancy and remove noisy detections. The combination of these features is the basis for the proposed architecture.

==> formatting/bibliography-setup.tex <==
\bibliography{ref} 
\bibliographystyle{ieeetr}

==> formatting/do_not_number.tex <==
%include this file in the preamble
%removes numbering from section headings
\setcounter{secnumdepth}{0} % sections are level 1

==> formatting/figures.tex <==
\newcommand{\fig}[3]
    {\begin{figure}
        \centering
        \includegraphics[width=#2in]{#1}
        \caption{#3}
        \label{#3}
     \end{figure}}


\newcommand{\tabl}[2]
    {\begin{table}
        \centering
        {#1}
        \caption{#2}
        \label{#2}
    \end{table}}
    
    
\newcommand{\figref}[1]{(Figure \ref{#1})}

\newcommand{\tableref}[1]{(Table \ref{#1})}

==> formatting/graphics.tex <==
%include this file in the preamble
%Adds images stored in the main file tree
%to use, "\includegraphics{fname.png}[]
\usepackage{graphicx}
\graphicspath{./}

==> formatting/header_footer.tex <==
\usepackage{fancyhdr}
\pagestyle{fancy}
\fancyhf{}
% \thepage inserts the page number
% [RE, RO] are alignment tabs
% \fancyfoot is also a command 
\fancyhead[RE,RO]{Advertisement Analysis: Surfrider Foundation \thepage}
\renewcommand{\headrulewidth}{0pt}

==> formatting/line_spacing.tex <==
\usepackage{setspace}
%set to 1 for single space, 2 for double space, and so on
\setstretch{1.5}

==> formatting/margins.tex <==
\usepackage[margin=0.5in]{geometry}

==> formatting/table_of_contents_setup.tex <==

%include this file in the preamble
%to use, type in "\tableofcontents" sometime after \begin{document}
\usepackage{color}   %May be necessary if you want to color links
\usepackage{hyperref}
\hypersetup{
    colorlinks=true, %set true if you want colored links
    linktoc=all,     %set to all if you want both sections and subsections linked
    linkcolor=blue,  %choose some color if you want links to stand out
}

==> sections/8_references.tex <==
\printbibliography
